The equivalence of information-theoretic and likelihood-based methods for neural dimensionality reduction

Stimulus dimensionality-reduction methods in neuroscience seek to identify a low-dimensional space of stimulus features that affect a neuron's probability of spiking. One popular method, known as maximally informative dimensions (MID), uses an information-theoretic quantity known as "single-spike information" to identify this space. Here we examine MID from a model-based perspective. We show that MID is a maximum-likelihood estimator for the parameters of a linear-nonlinear-Poisson (LNP) model, and that the empirical single-spike information corresponds to the normalized log-likelihood under a Poisson model. This equivalence implies that MID does not necessarily find maximally informative stimulus dimensions when spiking is not well described as Poisson. We provide several examples to illustrate this shortcoming, and derive a lower bound on the information lost when spiking is Bernoulli in discrete time bins. To overcome this limitation, we introduce model-based dimensionality reduction methods for neurons with non-Poisson firing statistics, and show that they can be framed equivalently in likelihood-based or information-theoretic terms. Finally, we show how to overcome practical limitations on the number of stimulus dimensions that MID can estimate by constraining the form of the non-parametric nonlinearity in an LNP model. We illustrate these methods with simulations and data from primate visual cortex.

==> mydefs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% Helpful definitions for TeX
%%%  Eero Simoncelli, 6/90.
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\long\def\comment#1{}
\long\def\nocomment#1{#1}   %to easily re-insert commented text
\long\def\mcomment#1{
	\marginpar[\singlesp\footnotesize #1 \fbox{\rule{1ex}{0ex}\rule{0ex}{1ex}}]
		  {\singlesp\footnotesize \fbox{\rule{1ex}{0ex}\rule{0ex}{1ex}} #1}}

%%% Set the spacing between lines: 1.0 means single-space.
%%% Must call a textsize command to get the new baselinestretch to
%%% work.  Thus this function resets the text size to \normalsize.
\def\setspacing#1{\renewcommand\baselinestretch{#1}\large\normalsize}

%%%  Use before 1st paragraph of a section to force an indentation.
%%% Correct solution is to redefine the sectioning commands in the
%%% appropriate style files (eg, art11.sty).
\newcommand{\yesindent}{\hspace*{\parindent}}    %%{\hskip \parindent}

\newcommand\doublesp{\renewcommand\baselinestretch{1.8}\large\normalsize}
\newcommand\singlesp{\renewcommand\baselinestretch{1.1}\large\normalsize}
\newcommand\halfsp{\renewcommand\baselinestretch{1.5}\large\normalsize}

\newenvironment{ct}
	{\begin{center}\begin{tabular}}
	{\end{tabular}\end{center}}

%%% Non-numbered subsections, with table of contents entries
\def\mychapter#1{\def\baselinestretch{1.0}\chapter{#1}\vskip 0.25in}
\def\mychap#1{\addcontentsline{toc}{chapter}{#1}
		\def\baselinestretch{1.0}\chapter*{#1}\vskip 0.25in}
\def\mysec#1{\addcontentsline{toc}{section}{$\circ$\hskip 0.4em #1}
		\section*{#1}}
\def\mysubsec#1{\addcontentsline{toc}{subsection}{$\circ$\hskip 0.4em #1} 
		\subsection*{#1}}
\def\mysubsubsec#1{\addcontentsline{toc}{subsubsection}{$\circ$\hskip 0.4em #1}
		\subsubsection*{#1}}

%%% A macro for figures to be MANUALLY pasted.  The arguments are the figure
%%% height, the figure label, and the figure caption.  The macro makes
%%% space for the figure, prints the label in center of the space (as
%%% an identifier), and prints the caption.
\long\def\myfig#1#2#3{
	\vbox to #1{\vfil \center{#2} \vfil} %Print label in box
	\caption{#3}
	\label{#2}}

%%% Macro for vertically aligning a subfigure and its label.
%%% Example usage: \sublabel{(a)}{\psfig{ ... }}
\def\sublabel#1#2{ \begin{tabular}{c} #2 \\  #1 \end{tabular}}

%%% New version of \caption puts things in smaller type, single-spaced 
%%% and indents them to set them off more from the text.
\makeatletter
\long\def\@makecaption#1#2{
	\vskip 0.8ex
	\setbox\@tempboxa\hbox{\small {\bf #1:} #2}
        \parindent 1.5em  %% How can we use the global value of this???
	\dimen0=\hsize
	\advance\dimen0 by -3em
	\ifdim \wd\@tempboxa >\dimen0
		\hbox to \hsize{
			\parindent 0em
			\hfil 
			\parbox{\dimen0}{\def\baselinestretch{0.96}\small
				{\bf #1.} #2
				%%\unhbox\@tempboxa
				} 
			\hfil}
	\else \hbox to \hsize{\hfil \box\@tempboxa \hfil}
	\fi
	}
\makeatother

%%%% original version of caption
%\long\def\@makecaption#1#2{
%   \vskip 10pt 
%   \setbox\@tempboxa\hbox{#1: #2}  
%   \ifdim \wd\@tempboxa >\hsize   % IF longer than one line:
%       \unhbox\@tempboxa\par      %   THEN set as ordinary paragraph.
%     \else                        %   ELSE  center.
%       \hbox to\hsize{\hfil\box\@tempboxa\hfil}  
%   \fi}

%%% Footnotes without numbers, modified from latex.tex definition of
%%% footnotetext.  NOTE: Can use \thanks if doing this on the title
%%% page. 
\makeatletter
\long\def\barenote#1{
    \insert\footins{\footnotesize
    \interlinepenalty\interfootnotelinepenalty 
    \splittopskip\footnotesep
    \splitmaxdepth \dp\strutbox \floatingpenalty \@MM
    \hsize\columnwidth \@parboxrestore
    {\rule{\z@}{\footnotesep}\ignorespaces
	      % indent
      #1\strut}}}
\makeatother

\def\bulletnote#1{\barenote{$\bullet$ #1}}
        
%%% Math definitions:
%\newtheorem{prop}{Proposition}
%\newenvironment{proof}{{\sl Proof: }}{\rule{0.07in}{0.13in}}

%%%p.100 Latex for \fbox with \rule
%%%Hollow: {\fbox{\rule{0.07in}{0in}\rule{0in}{0.14in}}}

%%% Inserting text into multi-line formulas.  See p. 193, Tex manual.
%%% Can also use \rm \noindent instead of \hbox, allowing longer lines.
%%\def\mtext#1{\noalign{\hbox{#1} \smallskip \medskip}}
\long\def\mtext#1{\noalign{\rm \noindent{#1}}}

%%% Insert space after or before or in an equation
%% \vbox to \medskipamount{\vfil}
%\def\eqsmallskip{\hbox{\smallskip }\nonumber\\}
%\def\eqmedskip{\hbox{\medskip} \nonumber \\}  
%\def\eqbigskip{\hbox{\bigskip} \nonumber \\} 
\def\eqsmallskip{\rule[\baselineskip]{0pt}{\smallskipamount}}
\def\eqmedskip{\rule[\baselineskip]{0pt}{\medskipamount}}
\def\eqbigskip{\rule[\baselineskip]{0pt}{\bigskipamount}}

%%% Alternative: use a strut (see p. 100 of LaTeX manual)

%%% Display fraction in textstyle (ie, with slash rather than
%%% horizontal bar)
\def\sfrac#1#2{{\textstyle \frac{#1}{#2}}}   

%% Format in tabbing (paragraph) mode, producing a box that is shrunk
%% to fit the paragraph.  First arg is margin, second is paragraph.
%% NOTE: minipage of tabbing fits paragraph, see LaTeX, p. 100.
\makeatletter
\long\def\shrinkbox{\@ifnextchar[{\@mgnshrinkbox}{\@shrinkbox}}

\def\@shrinkbox#1{
	\begin{minipage}{\columnwidth}\begin{tabbing}
	#1
	\end{tabbing}\end{minipage}}

\def\@mgnshrinkbox[#1]#2{
   \setbox\@tempboxa\hbox{\unskip\begin{minipage}{\columnwidth}\begin{tabbing}
		#2
		\end{tabbing}\end{minipage}\unskip}
   \dimen0=\wd\@tempboxa
   \advance\dimen0 by #1
   %%\advance\dimen0 by #1
   \dimen1=\ht\@tempboxa
   \advance\dimen1 by #1
   \advance\dimen1 by #1
   \makebox[\dimen0]{\vbox to \dimen1{\vfil \box\@tempboxa \vfil}}}
\makeatother

%  \F for the Fourieroperator
\newcommand{\F}{\mbox{$\cal F$}}

%  \R and \C   The set of Real and Complex numbers
%  may be used in equation or text mode
%  LaTeX has \Re but no \Co; define both in the traditional form (non script)
%\newcommand{\R}{\mbox{\rule[0ex]{.2ex}{1.56ex} \hspace{-1.6ex} \bf R}}
\newcommand{\R}{\mbox{I \hspace{-2ex} {\bf R}}} 
\newcommand{\C}{\mbox{   % mbox removes italics in equation mode
                \rule[.125ex]{0ex}{1.1ex}  % take out second line for now
                \hspace{-1.2ex}
                \rule[.0625ex]{.2ex}{1.4ex}
                \hspace{-2.4ex}
                \bf C
                }}
\newcommand{\Z}{\mbox{Z\hspace{-2ex}{\bf Z}}}

\def\etal{{\sl et~al.}}

%new caption macro
\makeatletter
\long\def\@makecaption#1#2{
        \vskip 10pt
        \setbox\@tempboxa\hbox{\small {\bf #1:} #2}
        \parindent 1.5em  %% How can we use the global value of this???
        \dimen0=\hsize
        \advance\dimen0 by -2\parindent
        \ifdim \wd\@tempboxa >\dimen0
                \hbox to \hsize{
                        \hfil
                        \parbox{\dimen0}{\def\baselinestretch{1.05}\small
                                {\bf #1:} #2
                                %%\unhbox\@tempboxa
                                }
                        \hfil}
        \else \hbox to \hsize{\hfil \box\@tempboxa \hfil}
        \fi}
\makeatother

% ============================================================
% More macros (jpdefs.tex)

\newcommand{\asection}[1]{
        \addtocounter{section}{1}
        \setcounter{subsection}{0}
        \section*{Appendix \Alph{section}: #1}
        \addcontentsline{toc}{section}{Appendix \Alph{section}: #1}}

\newcommand{\asubsection}[1]{
        \addtocounter{subsection}{1}
        \subsection*{\Alph{section}.\arabic{subsection} #1}
\addcontentsline{toc}{subsection}{\Alph{section}.\arabic{subsection} #1}}


\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}

% ---------- Symbols for ``Reals'', ``Complex Numbers'', etc. ----
\newcommand{\Reals}{{\sf R\hspace*{-0.9ex}\rule{0.15ex}%
{1.5ex}\hspace*{0.9ex}}}
\newcommand{\N}{{\sf N\hspace*{-1.0ex}\rule{0.15ex}%
{1.3ex}\hspace*{1.0ex}}}
\newcommand{\Q}{{\sf Q\hspace*{-1.1ex}\rule{0.15ex}%
{1.5ex}\hspace*{1.1ex}}}
\newcommand{\Complexs}{{\sf C\hspace*{-0.9ex}\rule{0.15ex}%
{1.3ex}\hspace*{0.9ex}}}

% ------- Others -------------------------------
\newcommand{\deriv}[2]{\frac{d #1}{d #2}}
\newcommand{\D}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\DD}[2]{\frac{\partial ^2 #1}{\partial #2 ^2}}
\newcommand{\Di}[2]{\frac{\partial ^i #1}{\partial #2 ^i}}
\newcommand{\evalat}[1]{\left.#1\right|}
\newcommand{\parderiv}[2]{\frac{\partial #1}{\partial{#2}}}
\newcommand{\parDeriv}[3]{\frac{\partial^{#3} #1}{\partial{#2}^{#3}}}
\newcommand{\parwrt}[1]{\frac{\partial}{\partial{#1}}}
\newcommand{\parpowrt}[2]{\frac{\partial^{#1}}{\partial {#2}^{#1}}}
\newcommand{\partwowrt}[2]{\frac{\partial^{2}}{\partial {#2} \partial{#1}}}
\newcommand{\parderivtwo}[3]{\frac{\partial^2 #1}{\partial{#2}\partial{#3}}}


